Sketch Decompositions for Classical Planning via Deep Reinforcement Learning

In planning and reinforcement learning, the identification of common subgoal structures across problems is important when goals are to be achieved over long horizons. Recently, it has been shown that such structures can be expressed as feature-based rules, called sketches, over a number of classical planning domains. These sketches split problems into subproblems which then become solvable in low polynomial time by a greedy sequence of IW$(k)$ searches. Methods for learning sketches using feature pools and min-SAT solvers have been developed, yet they face two key limitations: scalability and expressivity. In this work, we address these limitations by formulating the problem of learning sketch decompositions as a deep reinforcement learning (DRL) task, where general policies are sought in a modified planning problem where the successor states of a state s are defined as those reachable from s through an IW$(k)$ search. The sketch decompositions obtained through this method are experimentally evaluated across various domains, and problems are regarded as solved by the decomposition when the goal is reached through a greedy sequence of IW$(k)$ searches. While our DRL approach for learning sketch decompositions does not yield interpretable sketches in the form of rules, we demonstrate that the resulting decompositions can often be understood in a crisp manner.

==> sections/reproducibility.tex <==
\begin{figure*}

\section*{Reproducibility Checklist}

\begin{itemize}
    \item This paper:
    \begin{itemize}
        \item Includes a conceptual outline and/or pseudocode description of AI methods introduced. \textbf{(yes)}
        \item Clearly delineates statements that are opinions, hypotheses, and speculations from objective facts and results. \textbf{(yes)}
        \item Provides well-marked pedagogical references for less-familiar readers to gain background necessary to replicate the paper. \textbf{(yes)}
    \end{itemize}
    
    \item \textbf{Does this paper make theoretical contributions?} \textbf{(no)}
    \begin{itemize}
        \item If yes, please complete the list below:
        \begin{itemize}
            \item All assumptions and restrictions are stated clearly and formally. \textbf{(yes/partial/no)}
            \item All novel claims are stated formally (e.g., in theorem statements). \textbf{(yes/partial/no)}
            \item Proofs of all novel claims are included. \textbf{(yes/partial/no)}
            \item Proof sketches or intuitions are given for complex and/or novel results. \textbf{(yes/partial/no)}
            \item Appropriate citations to theoretical tools used are given. \textbf{(yes/partial/no)}
            \item All theoretical claims are demonstrated empirically to hold. \textbf{(yes/partial/no/NA)}
            \item All experimental code used to eliminate or disprove claims is included. \textbf{(yes/no/NA)}
        \end{itemize}
    \end{itemize}
    
    \item \textbf{Does this paper rely on one or more datasets?} \textbf{(no)}
    \begin{itemize}
        \item If yes, please complete the list below:
        \begin{itemize}
            \item A motivation is given for why the experiments are conducted on the selected datasets. \textbf{(yes/partial/no/NA)}
            \item All novel datasets introduced in this paper are included in a data appendix. \textbf{(yes/partial/no/NA)}
            \item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. \textbf{(yes/partial/no/NA)}
            \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. \textbf{(yes/no/NA)}
            \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available. \textbf{(yes/partial/no/NA)}
            \item All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisfying. \textbf{(yes/partial/no/NA)}
        \end{itemize}
    \end{itemize}
    
    \item \textbf{Does this paper include computational experiments?} \textbf{(yes)}
    \begin{itemize}
        \item If yes, please complete the list below:
        \begin{itemize}
            \item Any code required for pre-processing data is included in the appendix. \textbf{(yes)}
            \item All source code required for conducting and analyzing the experiments is included in a code appendix. \textbf{(yes)}
            \item All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. \textbf{(yes)}
            \item All source code implementing new methods has comments detailing the implementation, with references to the paper where each step comes from. \textbf{(yes)}
            \item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. \textbf{(yes)}
            \item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. \textbf{(yes)}
            \item This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. \textbf{(yes)}
            \item This paper states the number of algorithm runs used to compute each reported result. \textbf{(yes)}
            \item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. \textbf{(yes)}
            \item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). \textbf{(no)}
            \item This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. \textbf{(yes)}
            \item This paper states the number and range of values tried per (hyper-)parameter during development of the paper, along with the criterion used for selecting the final parameter setting. \textbf{(NA)}
        \end{itemize}
    \end{itemize}

\end{itemize}

\end{figure*}
